HADES: Microprocessor Hazard Analysis via Formal Verification of Parameterized Systems

HADES is a fully automated verification tool for pipeline-based microprocessors that aims at flaws caused by improperly handled data hazards. It focuses on single-pipeline microprocessors designed at the register transfer level (RTL) and deals with read-after-write, write-after-write, and write-after-read hazards. HADES combines several techniques, including data-flow analysis, error pattern matching, SMT solving, and abstract regular model checking. It has been successfully tested on several microprocessors for embedded applications.

==> eptcsdata.tex <==
\providecommand{\firstpage}{87}
\providecommand{\publicationstatus}{J. Bouda et al. (Eds.): 11th Doctoral Workshop\\
on  Mathematical and Engineering Methods\\
in Computer Science (MEMICS 2016)\\
EPTCS 233, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.233.9}{10.4204/EPTCS.233.9}}
\pdfoutput=1

